Foreign Object Detection and Quantification of Fat Content Using A Novel Multiplexing Electric Field Sensor

There is an ever growing need to ensure the quality of food and assess specific quality parameters in all the links of the food chain, ranging from processing, distribution and retail to preparing food. Various imaging and sensing technologies, including X-ray imaging, ultrasound, and near infrared reflectance spectroscopy have been applied to the problem. Cost and other constraints restrict the application of some of these technologies. In this study we test a novel Multiplexing Electric Field Sensor (MEFS), an approach that allows for a completely non-invasive and non-destructive testing approach. Our experiments demonstrate the reliable detection of certain foreign objects and provide evidence that this sensor technology has the capability of measuring fat content in minced meat. Given the fact that this technology can already be deployed at very low cost, low maintenance and in various different form factors, we conclude that this type of MEFS is an extremely promising technology for addressing specific food quality issues.

==> figures/coplanar.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(15816,3867)(418,-4144)
\thinlines
{\color[rgb]{0,.69,0}\put(6076,-3211){\framebox(900,2250){}}
}%
{\color[rgb]{0,.69,0}\put(9901,-3211){\framebox(6300,1800){}}
}%
{\color[rgb]{0,0,0}\put(7030,-2986){\vector( 0,-1){0}}
\put(6526,-2986){\oval(1008,360)[tr]}
\put(6526,-2986){\oval(1008,360)[tl]}
}%
{\color[rgb]{0,.69,0}\put(1351,-3211){\framebox(900,2700){}}
}%
{\color[rgb]{0,0,0}\put(1351,-2986){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(1351,-736){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(1351,-1486){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(1351,-2236){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(15976,-3211){\vector( 0,-1){0}}
\put(13051,-3211){\oval(5850,5850)[tr]}
\put(13051,-3211){\oval(5850,5850)[tl]}
}%
{\color[rgb]{0,0,0}\put(14476,-3211){\vector( 0,-1){0}}
\put(13051,-3211){\oval(2850,2850)[tr]}
\put(13051,-3211){\oval(2850,2850)[tl]}
}%
{\color[rgb]{0,0,0}\put(13726,-3211){\vector( 0,-1){0}}
\put(13051,-3211){\oval(1350,1350)[tr]}
\put(13051,-3211){\oval(1350,1350)[tl]}
}%
{\color[rgb]{0,0,0}\put(15225,-3211){\vector( 0,-1){0}}
\put(13051,-3211){\oval(4348,4348)[tr]}
\put(13051,-3211){\oval(4348,4348)[tl]}
}%
{\color[rgb]{0,0,0}\put(7516,-1486){\vector( 0,-1){0}}
\put(6515,-1486){\oval(2002,780)[tr]}
\put(6515,-1486){\oval(2002,780)[tl]}
}%
{\color[rgb]{0,0,0}\put(7291,-2236){\vector( 0,-1){0}}
\put(6526,-2236){\oval(1530,570)[tr]}
\put(6526,-2236){\oval(1530,570)[tl]}
}%
{\color[rgb]{0,0,0}\put(7786,-736){\vector( 0,-1){0}}
\put(6526,-736){\oval(2520,810)[tr]}
\put(6526,-736){\oval(2520,810)[tl]}
}%
\thicklines
{\color[rgb]{0,0,0}\put(2251,-1861){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(1351,-1861){\vector(-1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(14851,-3211){\vector( 0,-1){900}}
}%
{\color[rgb]{0,0,0}\put(16201,-3211){\line(-1, 0){2700}}
}%
{\color[rgb]{0,0,0}\put(11251,-3211){\vector( 0,-1){900}}
}%
{\color[rgb]{0,0,0}\put(9901,-3211){\line( 1, 0){2700}}
}%
{\color[rgb]{0,0,0}\put(5626,-1861){\vector(-1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(7426,-1861){\vector( 1, 0){900}}
}%
{\color[rgb]{0,0,0}\put(7876,-511){\line(-1,-3){900}}
}%
{\color[rgb]{0,0,0}\put(5176,-511){\line( 1,-3){900}}
}%
{\color[rgb]{0,0,0}\put(2251,-511){\line( 0,-1){2700}}
}%
{\color[rgb]{0,0,0}\put(1351,-511){\line( 0,-1){2700}}
}%
\end{picture}%

